Nested Session Types

Session types statically describe communication protocols between concurrent message-passing processes. Unfortunately, parametric polymorphism even in its restricted prenex form is not fully understood in the context of session types. In this paper, we present the metatheory of session types extended with prenex polymorphism and, as a result, nested recursive datatypes. Remarkably, we prove that type equality is decidable by exhibiting a reduction to trace equivalence of deterministic first-order grammars. Recognizing the high theoretical complexity of the latter, we also propose a novel type equality algorithm and prove its soundness. We observe that the algorithm is surprisingly efficient and, despite its incompleteness, sufficient for all our examples. We have implemented our ideas by extending the Rast programming language with nested session types. We conclude with several examples illustrating the expressivity of our enhanced type system.

==> dpda.tex <==
\section{Expressiveness of \PolymorphicSessionTypes}
\label{sec:dpdas}

\textbf{<to be rewritten>}

The polymorphic recursive nature underlying \polymorphicsessiontypes\ bears similarities with deterministic pushdown automata (DPDAs). In this section, we compare the expressiveness of \polymorphicsessiontypes\ with DPDAs and also with context-free session types.

The analysis of DPDAs usually distinguishes 
\emph{simple machines} from more expressive pushdown automata. A simple machine
is a DPDA with three additional properties~\cite{korenjak1966simple}:
\begin{enumerate}[label=(\roman*)]
	\item\label{itm:epsilon} has no $\varepsilon$-transitions;
	\item\label{itm:empty-stack}  accepts with empty stack;
	\item\label{itm:one-state}  has a single internal state.
\end{enumerate}

In this section we present a translation of polymorphic session types 
to DPDAs. We also see how the expressiveness of polymorphic session types
impact the properties stated above and which languages we can model
by relaxing them. Along the way, we will include an analysis of context-free
session types to complete the parallelism between session types and DPDAs 
and also to make explicit the distinctions between  polymorphic and context-free
session types.
Due to the contractiveness of session types, 
property~\ref{itm:epsilon} will not be relaxed.

\paragraph{Context-free session types~\cite{Thiemann16icfp}}
Context-free session types were introduced with the aim of releasing session types 
from tail recursion and enabling the necessary recursion 
to capture the expressiveness of (some) deterministic context-free 
grammars. 
Context-free session types can be translated into simple 
grammars~\cite{Almeida20tacas}, which means that there is a translation
of context-free session types into DPDAs satisfying the 
three properties stated above~\cite{korenjak1966simple}.

We can now wonder whether context-free session types coincide the unary case of 
polymorphic session types. The answer is no, although context-free session types
can be embedded into this fragment of polymorphic session types.
Recall the session type 
$\m{S}$ 
of strings from the language $\{\mb{a}^n\mb{b}^{n} \mid n > 0\}$ and
the corresponding context-free session type:

\begin{center}
  \begin{tabular}[t]{@{}l@{}}
    \emph{Context-free session type}
    \\ \midrule
    $   S' \triangleq \ichoice{\mb{a} : A' }$ 
    \\
    $   A' \triangleq \ichoice{\mb{a} : A';B',\enspace
     \mb{b} : \m{skip} }
    $ 
    \\
    $   B' \triangleq \ichoice{\mb{b} : \m{skip} }
    $ 
  \end{tabular}
  \qquad\qquad
  \begin{tabular}[t]{@{}l@{}}
    \emph{\Polymorphicsessiontype}
    \\ \midrule
    $    \m{S} \triangleq
      \ichoice{
        \mb{a} : \m{A}[\one]]
      }$
    \\
    $    \m{A}[\alpha] \triangleq
      \ichoice{
        \mb{a} : \m{A}[\m{B}[\alpha]],\enspace
        \mb{b} : \alpha
      }$
    \\
    $    \m{B}[\alpha] \triangleq
      \ichoice{
        \mb{b} : \alpha
      }$
  \end{tabular}
\end{center}

From this comparison, there is clearly a natural mapping between context-free session types and polymorphic session types
with unary type constructors.
Let $\mathcal{C}$ denote the set of context-free session types. We assume context-free 
session types are in a \emph{normal form} resulting
from applying the laws of sequential composition presented in Lemma 3.4 
of~\cite{Thiemann16icfp}, i.e., all redundant $\m{skip}$s are removed, the
distributive and associative laws are applied; we also assume recursive types
are defined through equations, $s \triangleq T$, rather than with the $\mu$ 
operator. Consider the 
transformation $\tau :\mathcal{C} \rightarrow \mathcal{T}$ defined as follows.
Each recursive definition is translated to a type constructor definition:
\begin{equation*}
  \tau(s \triangleq T) = (\m{s}[\alpha] \triangleq \tau_\alpha(T))
\end{equation*}
The body of the definition is translated with respect to a type parameter, $\alpha$, that represents the type of the continuation.
This auxiliary translation, indexed by a type parameter for the continuation, is given by:
\begin{equation*}
   \begin{array}[t]{lll}
       \tau_\alpha(\m{skip}) = \alpha\\
       \tau_\alpha(S;T) = [\tau_\alpha(T)/\beta]\tau_\beta(S)\\
       % \tau_\alpha(?\, B ) = \m B \tensor \alpha\\
       % \tau_\alpha(!\, B ) = \m B \lolli \alpha\smallskip\\
%       \tau_\alpha(?\, B ; S) = \m B \tensor \tau_\alpha(S)\\
%       \tau_\alpha(!\, B ; S) = \m B \lolli \tau_\alpha(S)\smallskip\\
    % \end{array}
    % \qquad
%    \begin{array}[t]{lll}
       \tau_\alpha(\ichoice{\ell : S_\ell}_{\ell\in L}) = \ichoice{\ell : \tau_\alpha({S}_\ell)}_{\ell\in L}\\
       \tau_\alpha(\echoice{\ell : S_\ell}_{\ell\in L}) = \echoice{\ell : \tau_\alpha({S}_\ell)}_{\ell\in L}\\
       \tau_\alpha(s) = \m{s}[\alpha]
    \end{array}
\end{equation*}
The first clause says that a context-free type $\m{skip}$ is translated to the type of a process that immediately calls its continuation of type $\alpha$.
In a sequential composition of context-free types, we first follow the translation of $S$, presuming that the continuation has type $\beta$, and the substitution $[\tau_{\alpha}(T)/\beta]$ ensures that that continuation type is precisely the type that corresponds to $T$.
The internal and external choice types simply push the continuation inside each branch of the choice.
And finally, recursive calls are translated to recursive calls to defined type constructors.

Notice that, under the above definitions for strings of the language $\{\mb{a}^n\mb{b}^n \mid n > 0\}$, we have $\tau(A' \triangleq\ichoice{\mb{a}:A';B', \mb{b}:\m{skip}}) = (\m{A}[\alpha] \triangleq \ichoice{\mb{a}:\m{A}[\m{B}[\alpha]],\mb{b}:\alpha})$ and $\tau(B' \triangleq \ichoice{\mb{b}:\m{skip}}) = (\m{B}[\alpha] \triangleq \ichoice{\mb{b}:\alpha})$ as desired.
However, the most natural translation of $S'$ would be $\tau(S' \triangleq \ichoice{\mb{a}:A'}) = (\m{S}'[\alpha] \triangleq \ichoice{\m{a}:\m{A}[\alpha]})$, which does not mathch the type $\m{S}$ exactly.
Nevertheless, $[\one/\alpha]\tau_\alpha(S') = \m{S}$, confirming that the difference between context-free session types and unary polymorphic session types is in the session termination 
operator: in context-free session types there is no way to abort a 
sequential composition in the middle of its execution and regardless 
of the continuation type, but in unary polymorphic session types there is.

The above translation also respects type equivalence on context-free session types: equivalent context-free types are translated to \emph{equal} unary polymophic session types.
As a simple example, $S;\m{skip}$ and $S$ are equivalent context-free types and $\tau_\alpha(S;\m{skip}) = [\alpha/\beta]\tau_{\beta}(S) = \tau_{\alpha}(S)$.

\paragraph{Unary polymorphic session types}
Endowed with the terminated session, unary polymorphic session types
can be translated into a DPDA accepting by final state (in contrast to 
acceptance by empty stack~\ref{itm:empty-stack}).
The translation to DPDAs can be obtained by considering:
\begin{itemize}
	\item the input alphabet $\Sigma$ resulting from all choice and
	send/receive actions 
	($\echoiceop\ell$, $\ichoiceop\ell$, $\tensor v$, $\lolli\ v$);
	\item the stack alphabet
$\Gamma$ containing the type names for all defined type constructors $\m{T}[x]$;
	\item the set of states $Q=\{q_0, q_a, q_r\}$, where $q_0$ is the initial state
	and $q_a$ is the only accept state;
	\item a transition function that, at $q_0$, given an input symbol $a$
	and a stack top symbol $\m{T}$, moves to $q_r$ if $a$ is not a valid action
	on $\m{T}[x]$; if $a$ is a valid action on $\m{T}[x]$ and denoting by 
	$\m{T}_a[x]$ the continuation of  $\m{T}[x]$ through $a$, the transition
	function is defined as follows:
	\begin{itemize}
		\item pops $\m{T}$ from the stack when reading $a$, 
		if $\m{T}_a[x]=x$,
		\item pops $\m{T}$ and pushes $\m{U_1}\ldots \m{U_n}$ onto the stack 
		when reading $a$, if $\m{T}_a[x] = \m{U_1}\cdots \m{U_n}[x]$,
		\item moves to the accept state $q_a$ when reading $a$, 
		if $\m{T}_a[x]=\one$.
	\end{itemize}
	All transitions from $q_r$ go to itself. Transitions from $q_a$ go to
	$q_r$.
\end{itemize}
We consider a preliminary step where we rewrite the type ensuring that:
(a) it starts with a defined type constructor rather than a 
built-in type constructor, (b) two built-in
type constructors always have intermediate defined type constructor(s),
and (c) the initial stack symbols are pushed onto the stack. 
To check that the input string $a_1\ldots a_m$ has type $\m{S_1}\cdots \m{S_n}[\m{A}]$,
we start pushing $\m{S_1}\ldots \m{S_n}\m{A}$ onto the stack.
Then, with input symbol $a_1$ and stack symbol $S_1$, we proceed
according to the transition function until consuming the input and
accepting or rejecting depending on the last state.

\paragraph{Polymorphic session types}
Polymorphic session types reflect, at the type level, the behavior of a DPDA.
These types lead to DPDAs with more than one internal state. 
The recognized languages are, thus, more expressive and relax 
properties~\ref{itm:empty-stack} and~\ref{itm:one-state} above.
Marvin Solomon defined a translation of types with polymorphic type 
constructors to DPDAs~\cite{Solomon78popl}. For the polymorphic types we propose,
and considering the input alphabet 
$\Sigma$ defined above, to check that the input string $a_1\ldots a_m$ has type 
$\m{S_1}\cdots \m{S_n}[\overline{\m{A}}]$, we can use the DPDA described below:
\begin{itemize}
	\item the stack alphabet $\Gamma$ is composed by symbols $S_{T,p}^U$ for each
	type constructor $U$ occurring in the type definition for $T$, at position $p$;
	\item the set of states $Q$ above is extended with states $q_\m{T}$ and $q_\m{Tx_i}$ 
	for each defined type constructor $\m{T}[\overline{x}]$ and type parameter
	$x_i$; it is also extended with auxiliary
	states needed for intermediate computations according to the
	interpretation of the type constructor at each projection;
	\item a transition function that: 
	\begin{itemize}
	\item in state $q_{\m{T}}$, with input symbol $a$, and stack
	symbol $T$, moves to $q_r$ if $a$ is not a valid action on $\m{T}[\overline{x}]$;
	otherwise, denoting by $\m{T}_a[\overline{x}]$ the continuation of 
	$\m{T}[\overline{x}]$ through $a$, the transition function is defined as follows, 
	when reading the input symbol $a$:
	\begin{itemize}
		\item if $\m{T}_a[\overline{x}]=\one$, moves to the accept 
		state $q_a$;
		\item if $\m{T}_a[\overline{x}]=x_i$, pops $T$ from the stack and then, reading the
		next stack symbol $S_{U,p}^V$, moves to state $q_{\m{Vx_i}}$, 
		\item if $\m{T}_a[\overline{x}] = \m{U}[\m{V}]$ 
		pops $T$ from the stack, pushes $S_{T,a}^U U$
		and moves to state $q_{U}$.
	\end{itemize}
	\item in state $q_{\m{Tx_i}}$, the automaton does not consume input; reading the 
	stack symbol $S_{U,p}^V$, and denoting by $V_{x_i}[\overline{x}]$ the projection
	of $V$ at the type definition $U$, position $p$, on the $i$-th argument, the
	transition function is defined as follows:
	\begin{itemize}
		\item if $V_{x_i}[\overline{x}] = x_j$, then pops $S_{U,p}^V$ from the stack
		and, if the next stack symbol is $S_{W,p}^Z$ moves to $q_{\m{Zx_j}}$, if the
		the next stack symbol is $T$, then moves to $q_\m{T}$;
		\item if $V_{x_i}[\overline{x}] = Z[W]$, then pops $S_{U,p}^V$ from the stack,
		pushes $S_{U,q}^Z Z$ onto the stack, and moves to $q_Z$;
	\end{itemize}
	\end{itemize}
	Transitions from $q_r$ go to itself. Transitions from $q_a$ go to $q_r$.
	For a given initial type $I \triangleq T[\overline{A}]$, the transition from 
	the initial state $q_0$ pushes $S_{I,1}^T T$ onto the stack. All the remaining
	transitions go to the reject state $q_r$.
\end{itemize}
As above, we consider a preliminary step consisting of rewriting the type and
ensuring it starts with a defined type constructor and that built-in 
type constructors are not nested. 








==> fig-lts-types.tex <==
%\begin{figure}[h]
  \begin{gather*}
  \frac{
  (\ell\in L)
  }{
  \ichoice{\ell : A_\ell}_{\ell\in L} \ltrans{\oplus \ell}{A_\ell} 
  }\ltsinchoice
  \enspace
    \frac{
  (\ell\in L)
  }{
  \echoice{\ell:A_\ell}_{\ell\in L}\ltrans{\& \ell}{A_\ell} 
  }\ltsextchoice
  \enspace
  \frac{
  %axiom
  }{
  A\tensor B \ltrans{\otimes A} B 
  }\ltstensor
  \enspace
  \frac{
  %axiom
  }{
  A \lolli B \ltrans{\multimap A} B 
  }\ltslolli
  \\\\  
  \frac{
      [\overline A / \overline x] B \ltrans{a} B'
      \quad
      (\m{T}[\overline x] \triangleq B) \in \Sigma
    }{
      \m{T}[\overline A] \ltrans{a} B'
    }\ltstypeconstr
  \end{gather*}
%  \caption{Labelled transition system for grounded polymorphic session types,
%  over a set of type definitions $\Sigma$.}
%  \label{fig:lts-session-types}
%\end{figure}

==> fig-syntax.tex <==
\begin{figure}[h]
  %
  \begin{align*}
  \m A \enspace &:: =   \enspace \ichoice{\ell : \m A}_{\ell\in L}
  \enspace | \enspace \echoice{\ell : \m A}_{\ell\in L} \enspace |\enspace \m A \tensor \m A \enspace | \enspace \m A \lolli \m A \enspace | \enspace \m T[\overline{\m A}] \enspace  | \enspace  \alpha \enspace | \enspace \one  
  \end{align*}
   Type definitions: $ \m T[\overline{\alpha}]= \m A$, where $A$ is contractive.
\caption{Syntax of polymorphic session types}
  \label{fig:session-types}
\end{figure}

==> macros-subtp.tex <==
\usepackage{stmaryrd} 
\usepackage{proof}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{mathtools}
\usepackage{amsthm}
\usepackage{mathpartir}
\usepackage{color}
\usepackage{xstring}


\newcommand{\W}{\Omega}
\newcommand{\Sg}{\Sigma}

\newcommand{\xvdash}[1]{%
  \vdash^{\mkern-10mu\scriptscriptstyle\rule[-.9ex]{0pt}{0pt}#1}%
}
\newcommand{\confpot}[2]{\overset{#1}{\underset{#2}{\vDash}}}
\newcommand{\potconf}[1]{\overset{#1}{\vDash}}
\newcommand{\spanconf}{\vDash}
\newcommand{\confspan}[1]{\overset{(#1)}{\vDash}}
\newcommand{\confspanlocal}[1]{\overset{\langle #1 \rangle}{\vDash}}
\newcommand{\D}{\Delta}
\newcommand{\G}{\Gamma}
\newcommand{\T}{\Theta}
\newcommand{\proves}{\vDash}


%% Proof Terms
\newcommand{\C}{\mathcal{C}}
\newcommand{\proc}[2]{\m{proc}(#1, #2)}
\newcommand{\msg}[2]{\m{msg}(#1, #2)}
\newcommand{\ichan}[3]{\m{ichan}(#1, #2, #3)}
\newcommand{\ochan}[3]{\m{ochan}(#1, #2, #3)}
\newcommand{\w}{\omega}
\newcommand{\ecase}[3]{\m{case} \; #1 \; (#2 \Rightarrow #3)}
\newcommand{\ecasecf}[3]{\m{case^{cf}} \; #1 \; (#2 \Rightarrow #3)}
\newcommand{\erecvch}[2]{#2 \leftarrow \m{recv} \; #1}
\newcommand{\erecvn}[2]{\{#2\} \leftarrow \m{recv} \; #1}
\newcommand{\erecvchcf}[2]{#2 \leftarrow \m{recv^{cf}} \; #1}
\newcommand{\erecvshift}[1]{\m{shift} \leftarrow \m{recv} \; #1}
\newcommand{\esendch}[2]{\m{send} \; #1 \; #2}
\newcommand{\esendn}[2]{\m{send} \; #1 \; \{#2\}}
\newcommand{\esendchcf}[2]{\m{send^{cf}} \; #1 \; #2}
\newcommand{\esendshift}[1]{\m{send} \; #1 \; \m{shift}}
\newcommand{\ewait}[1]{\m{wait} \; #1}
\newcommand{\ewaitcf}[1]{\m{wait^{cf}} \; #1}
\newcommand{\eclose}[1]{\m{close} \; #1}
\newcommand{\eclosecf}[1]{\m{close^{cf}} \; #1}
\newcommand{\fwd}[2]{#1 \leftarrow #2}
\newcommand{\fwdp}[2]{#1 \overset{+}{\leftarrow} #2}
\newcommand{\fwdn}[2]{#1 \overset{-}{\leftarrow} #2}
\newcommand{\m}[1]{\mathsf{#1}}
\newcommand{\esendl}[2]{#1.#2}
\newcommand{\esendlcf}[2]{(#1.#2)^{\m{cf}}}
\newcommand{\ecut}[4]{#1 \leftarrow #2 \leftarrow \overline{#3} \semi #4}
\newcommand{\espawn}[4]{#1 \leftarrow #2 \leftarrow #3 = #4}
\newcommand{\procg}[3]{\m{proc}(#1, #2, \overline{#3})}
\newcommand{\edelay}[1]{\m{delay} \; (#1)}
\newcommand{\ewhen}[2]{\m{when?} \; (#1) ; #2}
\newcommand{\enow}[2]{\m{now!} \; (#1) ; #2}
\newcommand{\etick}[1]{\m{tick} \; (#1)}
\newcommand{\ework}[1]{\m{work} \; \{#1\}}
\newcommand{\eget}[2]{\m{get} \; #1 \; \{#2\}}
\newcommand{\epay}[2]{\m{pay} \; #1 \; \{#2\}}
\newcommand{\procdef}[3]{#3 \leftarrow #1 \leftarrow #2}
\newcommand{\procdefna}[2]{#2 \leftarrow #1}
\newcommand{\casedef}[1]{\m{case} \; #1}
\newcommand{\labdef}[1]{#1 \Rightarrow}
\newcommand{\wk}[1]{\m{work}(#1)}
\newcommand{\eassume}[2]{\m{assume} \; #1 \; \{#2\}}
\newcommand{\eassert}[2]{\m{assert} \; #1 \; \{#2\}}
\newcommand{\eimpos}[2]{\m{impossible} \; #1 \; \{#2\}}
\newcommand{\imposs}{\m{impossible}}

%% Connnectives
\newcommand{\lolli}{\multimap}
\newcommand{\tensor}{\otimes}
\newcommand{\with}{\mathbin{\binampersand}}
\newcommand{\paar}{\mathbin{\bindnasrepma}}
\newcommand{\one}{\mathbf{1}}
\newcommand{\zero}{\mathbf{0}}
\newcommand{\bang}{{!}}
\newcommand{\whynot}{{?}}
\newcommand{\semi}{\; ; \;}
\newcommand{\ichoiceop}{\oplus}
\newcommand{\echoiceop}{\with}
\newcommand{\ichoice}[1]{\ichoiceop \{ #1 \}}
\newcommand{\echoice}[1]{\echoiceop \{ #1 \}}
\newcommand{\fuse}{\bullet}
\newcommand{\mi}[1]{\mbox{\it #1}}
\newcommand{\lunder}{\mathbin{\backslash}}
\newcommand{\tassertop}{?}
\newcommand{\tassumeop}{!}
\newcommand{\tassert}[1]{\; \tassertop\{#1\}. \;}
\newcommand{\tassume}[1]{\; \tassumeop\{#1\}. \;}

%% Potential
\newcommand{\pot}[2]{#1^{#2}}
\newcommand{\lollipot}[1]{\overset{#1}{\lolli}}
\newcommand{\tensorpot}[1]{\overset{#1}{\tensor}}
\newcommand{\potfop}{\phi}
\newcommand{\potf}[1]{\potfop(#1)}
\newcommand{\mlab}{M^{\textsf{label}}}
\newcommand{\mchan}{M^{\textsf{channel}}}
\newcommand{\mcl}{M^{\textsf{close}}}
\newcommand{\mall}{M}
\newcommand{\ms}{M_s}
\newcommand{\mr}{M_r}
\newcommand{\entailpot}[1]{\xvdash{#1}}
\newcommand{\entailpotcf}[1]{\underset{\m{cf}}{\entailpot{#1}}}
\newcommand{\entailspan}{\vdash}
\newcommand{\entailtype}{\vdash}
\newcommand{\fpot}{\; @ \;}
\newcommand{\pay}[1]{#1^{1}}
\newcommand{\sync}[1]{#1^{2}}
\newcommand{\spanpot}[1]{\langle \pay{#1}, \sync{#1} \rangle}
\newcommand{\ichoicepot}[2]{\overset{#1}{\ichoiceop} \{ #2 \}}
\newcommand{\echoicepot}[2]{\overset{#1}{\echoiceop} \{ #2 \}}
\newcommand{\tlist}[1]{\m{list}_{#1}}
\newcommand{\tdia}[1]{\Diamond #1}
\newcommand{\Dia}{\Diamond}
\newcommand{\tbox}[1]{\Box #1}
\newcommand{\tforall}[1]{\forall #1. \; }
\newcommand{\texists}[1]{\exists #1. \; }
\newcommand{\paypot}{\triangleright}
\newcommand{\getpot}{\triangleleft}
\newcommand{\tgetpot}[2]{\getpot^{#2} #1}
\newcommand{\tpaypot}[2]{\paypot^{#2} #1}
\newcommand{\indv}[1]{[\overline{#1}]}
\newcommand{\ind}[1]{\{#1\}}


%% Notation
\newcommand{\config}{\mathcal{C}}
\newcommand{\cost}[2]{\mathrm{cost}(\proc{#1}{#2})}
\newcommand{\tcost}[2]{\mathrm{cost}(#1 \mapsto #2)}
\newcommand{\ccost}[1]{\mathrm{cost}(#1)}
\newcommand{\dc}{\mathcal{D}}
\newcommand{\ec}{\mathcal{E}}
\newcommand{\ac}{\mathcal{A}}
\newcommand{\st}[1]{\m{store}_{#1}}
\newcommand{\stack}[1]{\m{stack}_{#1}}
\newcommand{\queue}[1]{\m{queue}_{#1}}
\newcommand{\mapper}[1]{\m{mapper}_{#1}}
\newcommand{\fdr}[1]{\m{folder}_{#1}}
\newcommand{\lt}[1]{\m{list}_{#1}}
\newcommand{\bits}{\m{bits}}
\newcommand{\ctr}{\m{ctr}}
\newcommand{\trans}[2]{#1 \Longrightarrow #2}
\newcommand{\delay}[2]{\left[#1\right]_{#2}}
\newcommand{\Next}{\raisebox{0.3ex}{$\scriptstyle\bigcirc$}}
\newcommand{\next}[1]{\Next #1}
\newcommand{\tdelay}[2]{
    \IfEqCase{#2}{%
        {1}{\next{#1}}%
        % you can add more cases here as desired
    }[{\Next^{#2} (#1)}]%
}%
\newcommand{\tock}[1]{`#1}
\newcommand{\sch}[1]{\tau(#1)}
\newcommand{\lforce}[2]{[#1]_L^{#2}}
\newcommand{\rforce}[2]{[#1]_R^{#2}}
\newcommand{\force}[2]{#1 \circ (#2)}
\newcommand{\typetrans}[1]{\left\lvert{#1}\right\rvert}
\newcommand{\tree}{\m{tree}}
\newcommand{\bool}{\m{bool}}
\newcommand{\true}{\top}
\newcommand{\false}{\bot}
\newcommand{\delayedbox}[1]{#1 \; \m{delayed}^{\Box}}
\newcommand{\delayeddia}[1]{#1 \; \m{delayed}^{\Diamond}}
\newcommand{\dom}[1]{\m{dom}(#1)}
\newcommand{\valid}[1]{#1 \; \m{valid}}

%% Subtyping
\newcommand{\subt}[2]{#1 \leq #2}
\newcommand{\wsubt}{ <: }
\newcommand{\qsubt}[1]{\overset{#1}{\leq}}

\newcommand{\impos}{\; \m{imposs}}
\newcommand{\unsat}{\; \m{unsat}}

\newcommand{\cons}{\mathcal{C}}
\newcommand{\vars}{\mathcal{V}}
\newcommand{\Vars}{\mathcal{V}}
\newcommand{\Cons}{\mathcal{C}}
\newcommand{\cmp}[4]{#1 \Vdash #2 \sim #3 = #4}
\newcommand{\unfldsg}[2]{\m{unfold}_{#1}(#2)}
\newcommand{\unfold}[1]{\unfldsg{\Sg}{#1}}
\newcommand{\rel}{\mathcal{R}}
\newcommand{\concs}[2]{\mathtt{clo}(#1) = #2}
\newcommand{\clo}[2]{\langle #1 \semi #2\rangle}

%% Latex
\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{cor}{Corollary}

%%Semantics
\newcommand{\step}{\mapsto}
\newcommand{\zerostep}{\step^{0}}
\newcommand{\mc}{\mathbf{c}}
\newcommand{\timed}[2]{\{#1\}_{#2}}
\newcommand{\unit}{M}
\newcommand{\Step}{\Longrightarrow}
\newcommand{\info}{\mapsto}
\newcommand{\andin}{\; \m{and} \;}
\newcommand{\minus}{\setminus}
\newcommand{\fresh}[1]{(#1 \text{ fresh})}

%%Global Semantics
\newcommand{\sinfer}[3]
{\inferrule
{#3}
{#2}
#1}
\newcommand{\enq}[2]{\m{enq}(#1, #2)}
\newcommand{\deq}[1]{\m{deq}(#1)}
\newcommand{\nil}{[]}
\newcommand{\elem}[1]{[#1]}

%% Channel typing
\newcommand{\eqdef}{\cong}

%% Types to Processes
\newcommand{\typeProc}[2]{#1 \Longrightarrow #2}

%% Configuration
\newcommand{\conftree}[3]{\left[#1\right] \; \proc{#2}{#3}}
\newcommand{\confprovider}[2]{(#1)^{#2}}
\newcommand{\confset}[1]{\overline{#1}}

%% Two Counter Machines
\newcommand{\ins}{\iota}
\newcommand{\tcm}{\mathcal{M}}
\newcommand{\inc}[1]{\m{inc}(#1)}
\newcommand{\dec}[1]{\m{dec}(#1)}
\newcommand{\goto}{\m{goto}}
\newcommand{\zeroc}[1]{\m{zero}(#1) ?}
\newcommand{\halt}{\m{halt}}

%% Reconstruction
\newcommand{\recon}[2]{#1 \Rightarrow #2}
\newcommand{\focus}[1]{[#1]}
\newcommand{\phiL}[1]{[#1]^{?}_L}
\newcommand{\phiR}[1]{[#1]^{!}_R}
\newcommand{\tpL}[1]{[#1]^{\tau}_L}
\newcommand{\tpR}[1]{[#1]^{\tau}_R}

%% Variance
\newcommand{\cov}{+}
\newcommand{\conv}{-}
\newcommand{\biv}{\bot}
\newcommand{\nonv}{\top}
\newcommand{\ofv}{\mathrel{\mbox{\tt\#}}}

==> macros-tmp.tex <==
\usepackage{stmaryrd} 
\usepackage{proof}
\usepackage{amsmath}
\usepackage{mathtools}
\usepackage{amsthm}
\usepackage{mathpartir}
\usepackage{color}
\usepackage{xstring}
\usepackage{ntabbing}
\usepackage{listings}
\usepackage{varwidth}
\usepackage{enumitem}
\usepackage{multicol}
\usepackage{lipsum}
\usepackage{booktabs}
\usepackage{subcaption}
\usepackage{fancyvrb}

\lstset{basicstyle=\ttfamily, columns=fullflexible, aboveskip=2pt, belowskip=2pt}

%% Polymorphic Nested Session Types
\newcommand{\polymorphicsessiontypes}[0]{nested session types}
\newcommand{\polymorphicsessiontype}[0]{nested session type}
\newcommand{\Polymorphicsessiontypes}[0]{Nested session types}
\newcommand{\Polymorphicsessiontype}[0]{Nested session type}
\newcommand{\PolymorphicSessionTypes}[0]{Nested Polymorphic Session Types}
\newcommand{\transl}[0]{\m{transl}}

%Potential annotations
\newlength{\rWidth}

\newcommand{\funtype}[1]{%
    {\settowidth{\rWidth}{\ensuremath{#1}}%
        \;\ensuremath{{\xrightarrow{\hspace{\rWidth}}\hspace{-0.84\rWidth}}\!\!\!^%
         {#1}%{\BehindSubString{,}{#1} / \BeforeSubString{,}{#1}}%
         \hspace{0.2\rWidth}\;\;}}}


%% Notation
\newcommand{\m}[1]{\mathsf{#1}}
\newcommand{\mb}[1]{\mathbf{#1}}

\newenvironment{sill}{\begin{tabbing}}{\end{tabbing}}


%% Configuration
\newcommand{\conftree}[3]{\left[#1\right] \; \proc{#2}{#3}}
\newcommand{\confprovider}[2]{(#1)^{#2}}
\newcommand{\confset}[1]{\overline{#1}}
\newcommand{\esync}{\; \m{esync}}

%% Modes
\newcommand{\s}{\m{S}}
\renewcommand{\l}{\m{L}}
\newcommand{\p}{\m{P}}

\newcommand{\lang}[1]{\mathbf{L}(#1)}

%% Contexts and Typing Judgment
\newcommand{\W}{\Omega}
\newcommand{\Sg}{\Sigma}
\newcommand{\xvdash}[1]{%
  \vdash^{\mkern-8mu\scriptstyle\rule[-.9ex]{0pt}{0pt}#1}%
}
\newcommand{\xVdash}[1]{%
  \Vdash^{\mkern-8mu\scriptstyle\rule[-.9ex]{0pt}{0pt}#1}%
}
\newcommand{\confpot}[2]{\overset{#1}{\underset{#2}{\vDash}}}
\newcommand{\potconf}[1]{\overset{#1}{\Vdash}}
\newcommand{\spanconf}{\vDash}
\newcommand{\confspan}[1]{\overset{(#1)}{\vDash}}
\newcommand{\confspanlocal}[1]{\overset{\langle #1 \rangle}{\vDash}}
\newcommand{\D}{\Delta}
\newcommand{\G}{\Gamma}
\newcommand{\T}{\Theta}
\newcommand{\proves}{\vDash}
\newcommand{\w}{\omega}
\newcommand{\C}{\mathcal{C}}
\newcommand{\set}[1]{\lvert\lvert#1\rvert\rvert}

\newcommand{\lin}[1]{\m{lin}(\overline{#1})}
\newcommand{\shd}[1]{\m{shd}(\overline{#1})}
\newcommand{\slin}[1]{\m{slin}(\overline{#1})}
\newcommand{\plin}{\; \m{purelin}}

%% Operational Semantics Predicates
\newcommand{\proc}[2]{\m{proc}(#1, #2)}
\newcommand{\msg}[2]{\m{msg}(#1, #2)}
\newcommand{\ichan}[3]{\m{ichan}(#1, #2, #3)}
\newcommand{\ochan}[3]{\m{ochan}(#1, #2, #3)}
\newcommand{\unavail}[1]{\m{unavail}(#1)}

%% Semantics
\newcommand{\step}{\mapsto}
\newcommand{\zerostep}{\step^{0}}
\newcommand{\mc}{\mathbf{c}}
\newcommand{\timed}[2]{\{#1\}_{#2}}
\newcommand{\unit}{M}
\newcommand{\Step}{\Longrightarrow}
\newcommand{\info}{\mapsto}
\newcommand{\andin}{\; \m{and} \;}
\newcommand{\minus}{\setminus}
\newcommand{\fresh}[1]{(#1 \text{ fresh})}
\newcommand{\eval}[1]{\Downarrow_{#1}}

%% Expressions Semantics
\newcommand{\val}{\; \m{val}}

%% Expressions
\newcommand{\lam}[3]{\lambda #1 : #2 . M_x}
\newcommand{\inl}[1]{l \cdot #1}
\newcommand{\inr}[1]{r \cdot #1}
\newcommand{\case}[3]{\m{case} \; #1 \; (l \hookrightarrow #2, r \hookrightarrow #3)}
\newcommand{\pair}[2]{\left\langle #1, #2 \right\rangle}
\newcommand{\projl}[1]{#1 \cdot l}
\newcommand{\projr}[1]{#1 \cdot r}
\newcommand{\match}[4]{\m{match} \; #1 \; ([] \rightarrow #2, #3 \rightarrow #4)}
\newcommand{\eproc}[3]{\{#1 \leftarrow #2 \leftarrow #3\}}


%% Proof Terms
\newcommand{\ecase}[3]{\m{case} \; #1 \; (#2 \Rightarrow #3)}
\newcommand{\ecasecf}[3]{\m{case^{cf}} \; #1 \; (#2 \Rightarrow #3)}
\newcommand{\erecvch}[2]{#2 \leftarrow \m{recv} \; #1}
\newcommand{\erecvn}[2]{\{#2\} \leftarrow \m{recv} \; #1}
\newcommand{\erecvchcf}[2]{#2 \leftarrow \m{recv^{cf}} \; #1}
\newcommand{\erecvshift}[1]{\m{shift} \leftarrow \m{recv} \; #1}
\newcommand{\esendch}[2]{\m{send} \; #1 \; #2}
\newcommand{\esendn}[2]{\m{send} \; #1 \; \{#2\}}
\newcommand{\esendchcf}[2]{\m{send^{cf}} \; #1 \; #2}
\newcommand{\esendshift}[1]{\m{send} \; #1 \; \m{shift}}
\newcommand{\ewait}[1]{\m{wait} \; #1}
\newcommand{\ewaitcf}[1]{\m{wait^{cf}} \; #1}
\newcommand{\eclose}[1]{\m{close} \; #1}
\newcommand{\eclosecf}[1]{\m{close^{cf}} \; #1}
\newcommand{\fwd}[2]{#1 \leftrightarrow #2}
\newcommand{\fwdp}[2]{#1 \overset{+}{\leftarrow} #2}
\newcommand{\fwdn}[2]{#1 \overset{-}{\leftarrow} #2}
\newcommand{\esendl}[2]{#1.#2}
\newcommand{\esendlcf}[2]{(#1.#2)^{\m{cf}}}
\newcommand{\ecut}[4]{#1 \leftarrow #2 \; #3 \semi #4}
\newcommand{\espawn}[4]{#1 \leftarrow #2 \leftarrow #3 = #4}
\newcommand{\procg}[3]{\m{proc}(#1, #2, \overline{#3})}
\newcommand{\edelay}[1]{\m{delay} \, (#1)}
\newcommand{\ewhen}[2]{\m{when?} \, (#1) ; #2}
\newcommand{\enow}[2]{\m{now!} \, (#1) ; #2}
\newcommand{\etick}[1]{\m{tick} \, (#1)}
\newcommand{\ework}[1]{\m{work} \, \{#1\}}
\newcommand{\eget}[2]{\m{get} \, #1 \, \{#2\}}
\newcommand{\epay}[2]{\m{pay} \, #1 \, \{#2\}}
\newcommand{\procdef}[3]{#3 \leftarrow #1 \; #2}
\newcommand{\procdefna}[2]{#2 \leftarrow #1}
\newcommand{\casedef}[1]{\m{case} \; #1}
\newcommand{\labdef}[1]{#1 \Rightarrow}
\newcommand{\wk}[1]{\m{work}(#1)}
\newcommand{\eif}[1]{\m{if} \; (#1)}
\newcommand{\ethen}{\; \m{then} \; }
\newcommand{\eelse}{\m{else} \; }
\newcommand{\eassume}[2]{\m{assume} \; #1 \; \{#2\}}
\newcommand{\eassert}[2]{\m{assert} \; #1 \; \{#2\}}
\newcommand{\eimpos}[2]{\m{impossible} \; #1 \; \{#2\}}
\newcommand{\eimposs}{\m{impossible}}

%% Type Constructors
\newcommand{\lolli}{\multimap}
\newcommand{\tensor}{\otimes}
\newcommand{\with}{\mathbin{\binampersand}}
\newcommand{\paar}{\mathbin{\bindnasrepma}}
\newcommand{\one}{\mathbf{1}}
\newcommand{\zero}{\mathbf{0}}
\newcommand{\bang}{{!}}
\newcommand{\whynot}{{?}}
\newcommand{\semi}{\; ; \;}
\newcommand{\ichoiceop}{\oplus}
\newcommand{\echoiceop}{\with}
\newcommand{\ichoice}[1]{\ichoiceop \{ #1 \}}
\newcommand{\echoice}[1]{\echoiceop \{ #1 \}}
\newcommand{\fuse}{\bullet}
\newcommand{\mi}[1]{\mbox{\it #1}}
\newcommand{\lunder}{\mathbin{\backslash}}
\newcommand{\arrow}{\to}
\newcommand{\product}{\times}
\newcommand{\tassertop}{{?}}  % -fp was: ?
\newcommand{\tassumeop}{{!}}  % -fp was: !
\newcommand{\tassert}[1]{\tassertop\{#1\}. \,} % -fp was: \; \tassertop
\newcommand{\tassume}[1]{\tassumeop\{#1\}. \,} % -fp was: \; \tassumeop
\newcommand{\true}{\top}
\newcommand{\false}{\bot}

%% Functional Types
\newcommand{\tproc}[2]{\{#1 \leftarrow #2\}}

%% Types with Potential
\newcommand{\pot}[2]{#1^{#2}}
\newcommand{\lollipot}[1]{\overset{#1}{\lolli}}
\newcommand{\tensorpot}[1]{\overset{#1}{\tensor}}
\newcommand{\potfop}{\phi}
\newcommand{\potf}[1]{\potfop(#1)}
\newcommand{\mlab}{M^{\textsf{label}}}
\newcommand{\mchan}{M^{\textsf{channel}}}
\newcommand{\mcl}{M^{\textsf{close}}}
\newcommand{\mall}{M}
\newcommand{\mint}{M^{\textsf{internal}}}
\newcommand{\mval}{M^{\textsf{value}}}
\newcommand{\mshd}{M^{\textsf{share}}}
\newcommand{\ms}{M_s}
\newcommand{\mr}{M_r}
\newcommand{\entailpot}[1]{\xvdash{#1}}
\newcommand{\ivdash}{\; _i{\vdash}\;}
\newcommand{\exppot}[1]{\xVdash{#1}}
\newcommand{\paypot}{\triangleright}
\newcommand{\getpot}{\triangleleft}
\newcommand{\tgetpot}[2]{\getpot^{#2} #1}
\newcommand{\tpaypot}[2]{\paypot^{#2} #1}
\newcommand{\bigeval}[3]{#1 \Downarrow #2 \mid #3}
\newcommand{\share}{\curlyveedownarrow}


%% Temporal Types
\newcommand{\entailpotcf}[1]{\underset{\m{cf}}{\entailpot{#1}}}
\newcommand{\entailspan}{\vdash}
\newcommand{\entailtype}{\vdash}
\newcommand{\fpot}{\; @ \;}
\newcommand{\pay}[1]{#1^{1}}
\newcommand{\sync}[1]{#1^{2}}
\newcommand{\spanpot}[1]{\langle \pay{#1}, \sync{#1} \rangle}
\newcommand{\ichoicepot}[2]{\overset{#1}{\ichoiceop} \{ #2 \}}
\newcommand{\echoicepot}[2]{\overset{#1}{\echoiceop} \{ #2 \}}
\newcommand{\tlist}[1]{\m{list}_{#1}}
\newcommand{\plist}[2]{L^{#2}(#1)}
\newcommand{\tdia}[1]{\Diamond #1}
\newcommand{\tbox}[1]{\Box #1}
\newcommand{\tforall}[1]{\forall #1. \, }
\newcommand{\texists}[1]{\exists #1. \, }
\newcommand{\delay}[2]{\left[#1\right]_{#2}}
\newcommand{\Next}{\raisebox{0.3ex}{$\scriptstyle\bigcirc$}}
% \newcommand{\next}[1]{\Next #1}
\newcommand{\tdelay}[2]{
    \IfEqCase{#2}{%
        {1}{\next{#1}}%
        % you can add more cases here as desired
    }[{\Next^{#2} (#1)}]%
}%
\newcommand{\tock}[1]{`#1}
\newcommand{\sch}[1]{\tau(#1)}
\newcommand{\lforce}[2]{[#1]_L^{#2}}
\newcommand{\rforce}[2]{[#1]_R^{#2}}
\newcommand{\force}[2]{#1 \circ (#2)}


%% Indices
\newcommand{\indv}[1]{\overline{[#1]}}
\newcommand{\ind}[1]{[#1]}


%% Syntactic Sugar
\newcommand{\config}{\mathcal{S}}
\newcommand{\cost}[2]{\mathrm{cost}(\proc{#1}{#2})}
\newcommand{\tcost}[2]{\mathrm{cost}(#1 \mapsto #2)}
\newcommand{\ccost}[1]{\mathrm{cost}(#1)}
\newcommand{\dc}{\mathcal{D}}
\newcommand{\ec}{\mathcal{E}}
\newcommand{\ac}{\mathcal{A}}
\newcommand{\st}[1]{\m{store}_{#1}}
\newcommand{\stack}[1]{\m{stack}_{#1}}
\newcommand{\queue}[1]{\m{queue}_{#1}}
\newcommand{\qu}[1]{\m{qu}_{#1}}
\newcommand{\mapper}[1]{\m{mapper}_{#1}}
\newcommand{\fdr}[1]{\m{folder}_{#1}}
\newcommand{\lt}[1]{\m{list}_{#1}}
\newcommand{\bits}{\m{bits}}
\newcommand{\ctr}{\m{ctr}}
\newcommand{\trans}[2]{#1 \Longrightarrow #2}
\newcommand{\typetrans}[1]{\left\lvert{#1}\right\rvert}
\newcommand{\tree}{\m{tree}}
\newcommand{\bool}{\m{bool}}
\newcommand{\delayedbox}[1]{#1 \; \m{delayed}^{\Box}}
\newcommand{\delayeddia}[1]{#1 \; \m{delayed}^{\Diamond}}
\newcommand{\dom}[1]{\m{dom}(#1)}
\newcommand{\valid}[1]{#1 \; \m{valid}}

%% Color
\newcommand{\B}[1]{\textcolor{blue}{#1}}
\newcommand{\R}[1]{\textcolor{red}{#1}}

%% Smart Contracts
\newcommand{\addr}{\m{addr}}
\newcommand{\ether}{\m{ether}}
\newcommand{\players}{\m{players}}
\newcommand{\lottery}{\m{lottery}}
\newcommand{\tint}{\m{int}}
\newcommand{\ballot}{\m{ballot}}
\newcommand{\tbool}{\m{bool}}
\newcommand{\lc}{\tlist{\m{coin}}}
\newcommand{\auction}{\m{auction}}
\newcommand{\object}{\m{object}}
\newcommand{\plcoin}{\m{plcoin}}
\newcommand{\plcoins}{\m{plcoins}}
\newcommand{\plcoinsn}{pl coins}

%% Typing Judgments for Servers and Clients
\newcommand{\sentailpot}[1]{\prescript{}{S}{\xvdash{#1}} \hspace{2pt}}
\newcommand{\centailpot}[1]{\prescript{}{C}{\xvdash{#1}} \hspace{2pt}}


%% Sharing
\newcommand{\down}{\downarrow^{\m{S}}_{\m{L}}}
\newcommand{\up}{\uparrow^{\m{S}}_{\m{L}}}
\newcommand{\eacquire}[2]{#1 \leftarrow \m{acquire} \; #2}
\newcommand{\eaccept}[2]{#1 \leftarrow \m{accept} \; #2}
\newcommand{\erelease}[2]{#1 \leftarrow \m{release} \; #2}
\newcommand{\edetach}[2]{#1 \leftarrow \m{detach} \; #2}


%% Subtyping
\newcommand{\subt}[2]{#1 \leq #2}
\newcommand{\wsubt}{ <: }
\newcommand{\qsubt}[1]{\overset{#1}{\leq}}

\newcommand{\impos}{\; \m{imposs}}
\newcommand{\imposs}{\m{impossible}}
\newcommand{\unsat}{\; \m{unsat}}

\newcommand{\cons}{\mathcal{C}}
\newcommand{\vars}{\mathcal{V}}
\newcommand{\Vars}{\mathcal{V}}
\newcommand{\Cons}{\mathcal{C}}

\newcommand{\cmp}[4]{#1 \Vdash #2 \sim #3 = #4}

\newcommand{\unfldsg}[2]{\m{unfold}_{#1}(#2)}
\newcommand{\unfold}[1]{\unfldsg{\Sg}{#1}}
\newcommand{\rel}{\mathcal{R}}
\newcommand{\concs}[2]{\mathtt{conc}(#1) = #2}


%% Latex
\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{cor}{Corollary}


%%Global Semantics
\newcommand{\sinfer}[3]
{\inferrule
{#3}
{#2}
#1}
\newcommand{\enq}[2]{\m{enq}(#1, #2)}
\newcommand{\deq}[1]{\m{deq}(#1)}
\newcommand{\nil}{[]}
\newcommand{\elem}[1]{[#1]}


%% Channel typing
\newcommand{\eqdef}{\cong}


%% Types to Processes
\newcommand{\typeProc}[2]{#1 \Longrightarrow #2}

%% Solidity
\definecolor{verylightgray}{rgb}{.97,.97,.97}

\lstdefinelanguage{Solidity}{
	keywords=[1]{anonymous, assembly, assert, balance, break, call, callcode, case, catch, class, constant, continue, constructor, contract, debugger, default, delegatecall, delete, do, else, emit, event, experimental, export, external, false, finally, for, function, gas, if, implements, import, in, indexed, instanceof, interface, internal, is, length, library, log0, log1, log2, log3, log4, memory, modifier, new, payable, pragma, private, protected, public, pure, push, require, return, returns, revert, selfdestruct, send, solidity, storage, struct, suicide, super, switch, then, this, throw, transfer, true, try, typeof, using, value, view, while, with, addmod, ecrecover, keccak256, mulmod, ripemd160, sha256, sha3}, % generic keywords including crypto operations
	keywordstyle=[1]\color{blue}\bfseries,
	keywords=[2]{address, bool, byte, bytes, bytes1, bytes2, bytes3, bytes4, bytes5, bytes6, bytes7, bytes8, bytes9, bytes10, bytes11, bytes12, bytes13, bytes14, bytes15, bytes16, bytes17, bytes18, bytes19, bytes20, bytes21, bytes22, bytes23, bytes24, bytes25, bytes26, bytes27, bytes28, bytes29, bytes30, bytes31, bytes32, enum, int, int8, int16, int24, int32, int40, int48, int56, int64, int72, int80, int88, int96, int104, int112, int120, int128, int136, int144, int152, int160, int168, int176, int184, int192, int200, int208, int216, int224, int232, int240, int248, int256, mapping, string, uint, uint8, uint16, uint24, uint32, uint40, uint48, uint56, uint64, uint72, uint80, uint88, uint96, uint104, uint112, uint120, uint128, uint136, uint144, uint152, uint160, uint168, uint176, uint184, uint192, uint200, uint208, uint216, uint224, uint232, uint240, uint248, uint256, var, void, ether, finney, szabo, wei, days, hours, minutes, seconds, weeks, years},	% types; money and time units
	keywordstyle=[2]\color{teal}\bfseries,
	keywords=[3]{block, blockhash, coinbase, difficulty, gaslimit, number, timestamp, msg, data, gas, sender, sig, value, now, tx, gasprice, origin},	% environment variables
	keywordstyle=[3]\color{violet}\bfseries,
	identifierstyle=\color{black},
	sensitive=false,
	comment=[l]{//},
	morecomment=[s]{/*}{*/},
	commentstyle=\color{gray}\ttfamily,
	stringstyle=\color{red}\ttfamily,
	morestring=[b]',
	morestring=[b]"
}

%% Focusing
\newcommand{\recon}[2]{#1 \Rightarrow #2}
\newcommand{\focus}[1]{[#1]}
\newcommand{\phiL}[1]{[#1]^{?}_L}
\newcommand{\phiR}[1]{[#1]^{!}_R}
\newcommand{\tpL}[1]{[#1]^{\tau}_L}
\newcommand{\tpR}[1]{[#1]^{\tau}_R}

%% Two Counter Machines
\newcommand{\ins}{\iota}
\newcommand{\tcm}{\mathcal{M}}
\newcommand{\inc}[1]{\m{inc}(#1)}
\newcommand{\dec}[1]{\m{dec}(#1)}
\newcommand{\goto}{\m{goto}}
\newcommand{\zeroc}[1]{\m{zero}(#1) ?}
\newcommand{\halt}{\m{halt}}

%% Type Equivalence Polymorphism
\newcommand{\typevars}{\mathcal{V}}
\newcommand{\optlabel}{\%}
\newcommand{\ltrans}[1]{\xrightarrow{#1}}
\newcommand{\opt}[1]{#1_{\optlabel}}

\newcommand{\clo}[2]{\langle #1 \semi #2\rangle}

%% Labelled Transition System
\newcommand{\ltsinchoice}{\m{LT}\ichoiceop}
\newcommand{\ltsextchoice}{\m{LT}\echoiceop}
\newcommand{\ltstensor}{\m{LT}\tensor}
\newcommand{\ltslolli}{\m{LT}\lolli}
\newcommand{\ltstypeconstr}{\m{LT}[-]}



==> polymorphic-types.tex <==
\section{\PolymorphicSessionTypes}
\label{sec:polymorphic-types}

This section formalizes the syntax of polymorphic session types. 
By introducing type constructors and type parameters, polymorphic
session types enable the specification of polymorphic recursion
on session types.

\subsection{Syntax}

The syntax of polymorphic session types considers the usual session type operators for 
choice, channel passing and termination ($\ichoiceop$, $\echoiceop$, 
$\tensor$, $\lolli$, $\one$), but also 
type constructors $\m T [\overline \alpha]$, 
parameterized with type parameters $\overline \alpha$.
Figure~\ref{fig:session-types} summarizes the syntax of polymorphic session types. 

\input{fig-syntax}

We now overview the usual basic operators and the type definitions
underlying the syntax.
The \emph{internal choice} operator $\ichoice{\ell : \m A_{\ell}}_{\ell\in L}$ 
selects a branch over labels $\ell\in L$, with continuation types
$\m A_{\ell}$. The \emph{external choice} operator 
$\echoice{\ell : \m A_{\ell}}_{\ell\in L}$  offers a choice
with labels $\ell\in L$, providing continuation types
$\m A_{\ell}$. The \emph{tensor} operator $\m{A}\tensor\m{B}$ 
represents the channel passing type that consists in sending a
channel of type $\m{A}$ and proceeding with type $\m{B}$.
Dually, the operator $\m{A}\lolli\m{B}$ consists on 
receiving a channel of type $\m{A}$ and continuing with 
type $\m{B}$. The \emph{terminated session} $\one$ is
the operator that closes the session.

Polymorphic session types can also be defined through the application of type 
constructors $\m{T}[\overline{\m{A}}]$.
A \emph{type constructor} $\m{T}[\overline{\alpha}]$ 
is defined by means of type definitions 
$ \m{T}[\overline{\alpha}]\triangleq \m{A},$
where $\m{A}$ is a contractive type, i.e., it can be an 
internal/external choice, tensor, lolli, or $\one$.
Type constructors are parametrized with type parameters $\overline{\alpha}$,
that can be instantiated with types upon application. Type constructors with
a single type parameter are called \emph{unary type} constructors.
The type definitions underlying the syntax of polymorphic session types are
collected in a set $\Sigma$.


%
The set of free variables in a type $A$ is defined as usual, as well
as the substitution of types $\overline B$ 
for variables $\overline \alpha$ in $A$, 
represented by $[\overline B/\overline \alpha] A$.
We use $\mathcal{T}$ to refer to the set of ground polymorphic session types 
(without any free variable). 

\input{dpda}



==> tab_syntax.tex <==
\begin{table}
  \centering
  \begin{tabular}{l l l}
  \textbf{Abstract Type\quad} & \textbf{Concrete Type\quad} & \textbf{Concrete Syntax} \\
  \toprule
  $\texists{x} A$ & \verb|?[x]. A| & \verb|send x [B]| \\
  $\tforall{x} A$ & \verb|![x]. A| & \verb|[B] <- recv x| \\
  $V\indv{x}$ & \verb|V[x1]...[xk]| \\
  \bottomrule
  \end{tabular}
  \caption{Abstract and Corresponding Concrete Syntax}
  \label{tab:syntax}
  \vspace{-1.5em}
\end{table}
  
